Enhancing Code Generation Performance of Smaller Models by Distilling the Reasoning Ability of LLMs

Large Language Models (LLMs) have recently made significant advances in code generation through the 'Chain-of-Thought' prompting technique. This technique empowers the model to autonomously devise "solution plans" to tackle intricate programming challenges, thereby improving its performance in code generation. Nevertheless, smaller models have been struggling to keep up with LLMs in deducing these plans, adversely affecting their code generation capabilities. Given the considerable size and associated deployment costs, along with concerns about data security, many teams opt for deploying smaller models for code generation. Consequently, there arises a compelling need for transferring LLMs' code generation reasoning abilities to the smaller models. In this paper, we propose the CodePLAN framework, which aims to transfer LLMs' reasoning capabilities to smaller models through distillation. We adopt a multi-task learning approach, jointly undertaking code generation and solution plan generation tasks, to enhance the code generation capabilities of the smaller model. To ensure the superior quality of the solution plans, we advocate for the utilization of backward reasoning and plan sampling strategies. Our experiments show that in comparison to the conventional fine-tuning approach, our approach improves the smaller model's code generation performance (measured in pass@1 metric) by over 130% on the challenging APPS benchmark.

==> tabels/06_table_6.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
%\begin{wraptable}{r}{0.65\textwidth}
% \vspace{-0.1in}

\centering
%\small
\resizebox{0.95\textwidth}{!} {
\begin{tabular}{c|cccc|}
\hline
\multicolumn{1}{c|}{Method}   & \multicolumn{1}{c}{Intro}         & \multicolumn{1}{c}{Inter}         & \multicolumn{1}{c}{Comp}          & \multicolumn{1}{c}{All}   \\ 
\hline
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{CodeT5-770M\quad \quad \quad \quad Pass@1}} \\
\hline
\multicolumn{1}{c|}{No-Plan} & 3.30 & 0.68 & 0.16 & \multicolumn{1}{c}{1.10}  \\
\multicolumn{1}{c|}{With-Plan(greedy)} & $4.90 \ \ (\textcolor{red}{\uparrow 48.5\%})$ & $1.03 \ \ (\textcolor{red}{\uparrow 51.5\%})$ & $0.14 \ \ (\textcolor{blue}{\downarrow 14.3\%})$ & \multicolumn{1}{c}{$1.62 \ \ (\textcolor{red}{\uparrow 47.3\%})$} \\
\multicolumn{1}{c|}{With-Plan(best)} & $\textbf{9.72} \ \ (\textcolor{red}{\uparrow 194.5\%})$  & $\textbf{1.91} \ \ (\textcolor{red}{\uparrow 180.9\%})$  & $\textbf{0.45} \ \ (\textcolor{red}{\uparrow 181.3\%})$  & \multicolumn{1}{c}{$\textbf{3.18} \ \ (\textcolor{red}{\uparrow 189.1\%})$} \\
\hline
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{CodeT5-770M\quad \quad \quad \quad Pass@5}} \\
\hline
\multicolumn{1}{c|}{No-Plan} & 8.12 & 2.01 & 0.74 & \multicolumn{1}{c}{2.98}  \\
\multicolumn{1}{c|}{With-Plan(greedy)} & $11.30 \ \ (\textcolor{red}{\uparrow 39.2\%})$ & $2.69 \ \ (\textcolor{red}{\uparrow 33.8\%})$ & $0.61 \ \ (\textcolor{blue}{\downarrow 17.6\%})$ & \multicolumn{1}{c}{$4.00 \ \ (\textcolor{red}{\uparrow 34.2\%})$} \\
\multicolumn{1}{c|}{With-Plan(best)} & $\textbf{18.90} \ \ (\textcolor{red}{\uparrow 132.8\%})$  & $\textbf{4.56} \ \ (\textcolor{red}{\uparrow 126.9\%})$  & $\textbf{1.80} \ \ (\textcolor{red}{\uparrow 143.2\%})$  & \multicolumn{1}{c}{$\textbf{6.88} \ \ (\textcolor{red}{\uparrow 130.9\%})$} \\
\hline
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{CodeT5-220M\quad \quad \quad \quad Pass@1}} \\
\hline
\multicolumn{1}{c|}{No-Plan} & 0.71 & 0.27 & 0.03 & \multicolumn{1}{c}{0.31}  \\
\multicolumn{1}{c|}{With-Plan(greedy)} & $1.36 \ \ (\textcolor{red}{\uparrow 91.5\%})$ & $ 0.29 \ \ (\textcolor{red}{\uparrow 7.41\%})$ & $0.04 \ \ (\textcolor{red}{\uparrow 33.3\%})$ & \multicolumn{1}{c}{$0.45 \ \ (\textcolor{red}{\uparrow 45.2\%})$} \\
\multicolumn{1}{c|}{With-Plan(best)} & $\textbf{1.62} \ \ (\textcolor{red}{\uparrow 128.2\%})$  & $\textbf{0.40} \ \ (\textcolor{red}{\uparrow 48.2\%})$  & $\textbf{0.06} \ \ (\textcolor{red}{\uparrow 100.0\%})$  & \multicolumn{1}{c}{$\textbf{0.58} \ \ (\textcolor{red}{\uparrow 87.1\%})$} \\
\hline
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{CodeT5-220M\quad \quad \quad \quad Pass@5}} \\
\hline
\multicolumn{1}{c|}{No-Plan} & 2.40 & 0.94 & 0.12 & \multicolumn{1}{c}{1.07}  \\
\multicolumn{1}{c|}{With-Plan(greedy)} & $3.56 \ \ (\textcolor{red}{\uparrow 48.3\%})$ & $1.02 \ \ (\textcolor{red}{\uparrow 8.5\%})$ & $0.19 \ \ (\textcolor{red}{\uparrow 58.3\%})$ & \multicolumn{1}{c}{$1.36 \ \ (\textcolor{red}{\uparrow 27.1\%})$} \\
\multicolumn{1}{c|}{With-Plan(best)} & $\textbf{4.71} \ \ (\textcolor{red}{\uparrow 96.3\%})$  & $\textbf{1.22} \ \ (\textcolor{red}{\uparrow 29.8\%})$  & $\textbf{0.24} \ \ (\textcolor{red}{\uparrow 100.0\%})$  & \multicolumn{1}{c}{$\textbf{1.70} \ \ (\textcolor{red}{\uparrow 58.9\%})$} \\
\hline
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{GPT2-1.5B\quad \quad \quad \quad \quad \quad Pass@1}} \\
\hline
\multicolumn{1}{c|}{No-Plan} & 1.30 & \textbf{0.70} & 0.00 & \multicolumn{1}{c}{0.68}  \\
\multicolumn{1}{c|}{With-Plan(greedy)} & $3.37 \ \ (\textcolor{red}{\uparrow 159.2\%})$ & $0.50 \ \ (\textcolor{blue}{\downarrow 40.0\%})$ & $0.04 \ \ (\textcolor{red}{\uparrow \infty})$ & \multicolumn{1}{c}{$0.94 \ \ (\textcolor{red}{\uparrow 38.2\%})$} \\
\multicolumn{1}{c|}{With-Plan(best)} & $\textbf{4.13} \ \ (\textcolor{red}{\uparrow 217.7\%})$  & $0.65 \ \ (\textcolor{blue}{\downarrow 7.1\%})$  & $\textbf{0.08} \ \ (\textcolor{red}{\uparrow \infty})$  & \multicolumn{1}{c}{$\textbf{1.20} \ \ (\textcolor{red}{\uparrow 76.5\%})$} \\
\hline
\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{GPT2-1.5B\quad \quad \quad \quad \quad \quad Pass@5}} \\
\hline
\multicolumn{1}{c|}{No-Plan} & 3.60 & 1.03 & 0.00 & \multicolumn{1}{c}{1.34}  \\
\multicolumn{1}{c|}{With-Plan(greedy)} & $8.20 \ \ (\textcolor{red}{\uparrow 127.8\%})$ & $1.54 \ \ (\textcolor{red}{\uparrow 49.5\%})$ & $0.22 \ \ (\textcolor{red}{\uparrow \infty})$ & \multicolumn{1}{c}{$2.51 \ \ (\textcolor{red}{\uparrow 87.3\%})$} \\
\multicolumn{1}{c|}{With-Plan(best)} & $\textbf{9.66} \ \ (\textcolor{red}{\uparrow 168.3\%})$  & $\textbf{1.79} \ \ (\textcolor{red}{\uparrow 73.8\%})$  & $\textbf{0.38} \ \ (\textcolor{red}{\uparrow \infty})$  & \multicolumn{1}{c}{$\textbf{3.02} \ \ (\textcolor{red}{\uparrow 125.4\%})$} \\
\hline
\end{tabular}
}
%\end{wraptable}
\caption{Results of different smaller models on APPS with different solution plans generated from LLM.} 
\label{tab: tabel6}
\end{table*}
